Search for supersymmetry in final states with two same sign leptons or three leptons and jets with the ATLAS detector at the LHC

The Standard Model of particle physics successfully describes the elementary particles and their interactions at low energies, up to 100 GeV. Beyond this scale lies the realm of new physics needed to remedy problems that arise at higher energies, the TeV scale and above. Supersymmetry (SUSY) is the most favored extension of the Standard Model that solves many of its limitations, if predicted SUSY particles exist at the TeV scale. The Large Hadron Collider (LHC) at CERN has opened a new phase of exploration into new physics at the TeV scale after increasing the center-of-mass energy of the proton-proton collisions to 13 TeV. The ATLAS experiment has collected this collision data with over 90% efficiency due to the excellent performance of many of its systems, in particular the data acquisition system. The work described in this dissertation ensures the efficient collection of ATLAS data as well as the analysis of this data to search for SUSY. The search for strongly produced supersymmetric particles decaying into final states with multiple energetic jets and either two leptons (electrons or muons) with the same electric charge or at least three leptons was performed using the proton-proton collision dataset of 36 fb$^{-1}$ at 13 TeV recorded with the ATLAS detector in 2015 and 2016. Due to the low Standard Model background, these final states are particularly adapted to searches for gluinos or third generation squarks in several supersymmetric production topologies determined from a variety of simplified and phenomenological models. The absence of excess over the Standard Model prediction is interpreted in terms of limits on the masses of superpartners derived at 95% confidence level. In the studied decay modes and depending on the decay topology, the existence of gluinos with masses below 1.9 TeV, sbottoms with masses below 700 GeV, and neutralinos with masses below 1.2 TeV are excluded.

==> texfiles/app.auxiliary.tex <==
%replaced \ninoone with \tilde\chi^0_1


\begin{figure}[htb!]
\centering
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{best_Rpc2L2b}\caption{}\label{fig:best_Rpc2L2b}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{best_Rpc2L0b}\caption{}\label{fig:best_Rpc2L0b}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{best_Rpc3L0b}\caption{}\label{fig:best_Rpc3L0b}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{best_Rpc2L1b}\caption{}\label{fig:best_Rpc2L1b}\end{subfigure}
\caption{Illustration of the best expected signal region per signal grid point for the 
$\gluino\to q\bar q (\ell\ell/\nu\nu)\tilde\chi^0_1$ (Fig.~\ref{fig:feynman_gtt}), $\gluino\to q\bar q' WZ\tilde\chi^0_1$ (Fig.~\ref{fig:feynman_gg2WZ}),
$\gluino\to q\bar q' \ell/\nu \ell/\nu \tilde\chi^0_1$ (Fig.~\ref{fig:feynman_gg2sl}), $\sbottom\to t W \tilde\chi^0_1$ (Fig.~\ref{fig:feynman_b1b1}) models. 
This mapping is used for the final combined exclusion limits.}
\label{fig:best_SR}
\end{figure}


\clearpage

\begin{figure}[p]
\centering
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{GreyNumbers/Gtt_SRbest}\caption{Rpc2L2bS/H, Rpc2Lsoft1b/2b}\label{fig:GN_limits_feynman_gtt}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{GreyNumbers/2stepWZ_SRbest}\caption{Rpc2L0bS, Rpc2L0bH}\label{fig:GN_limits_feynman_gg2WZ}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{GreyNumbers/GSL_SRbest.pdf}\caption{Rpc3L0bS, Rpc3L0bH}\label{fig:GN_limits_feynman_gg2sl}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{GreyNumbers/Btt_SRbest.pdf}\caption{Rpc2L1bS, Rpc2L1bH}\label{fig:GN_limits_feynman_b1b1}\end{subfigure}

\caption{Observed and expected exclusion limits on the $\tilde{g}$, \sbottomone, \stopone and \ninoone masses 
in the context of RPC SUSY scenarios with simplified mass spectra. The signal regions used to obtain the limits are specified in the subtitle of each scenario. All limits are computed at 95\% CL. The dotted lines around the observed
limit illustrate the change in the observed limit as the nominal signal cross-section is scaled up and down
by the theoretical uncertainty. The contours of the band around the expected 
limit are the $\pm$1$\sigma$ results, 
including all uncertainties except the theoretical ones on the signal cross-section. In 
Figures~\ref{fig:GN_limits_feynman_gtt}--\ref{fig:GN_limits_feynman_b1b1}, the grey diagonal lines indicate the kinematic limit for the decays in each 
specified scenario and results are compared with the observed limits obtained by previous ATLAS searches~\cite{paperSS3L,Aad:2016jxj}. 
The grey numbers show 95\% CL upper limits on production cross-sections (in fb) obtained using the signal efficiency and acceptance specific to each model.}
\label{fig:Results_Limits_RPC_GN} 
\end{figure} 

\clearpage

\begin{table}[ht]\centering\def\arraystretch{1.2}\begin{tabular}{|l|c|}\hline
   \multicolumn{2}{|l|}{Rpc2L2bS,\quad$\gluino\gluino$ production,\quad$\gluino\to \ttbar\ninoone$}\\
   \multicolumn{2}{|l|}{$m_{\gluino}= 1.5 \TeV$, $m_{\ninoone}= 800 \GeV$}\\\hline
   MC events generated  & 98000 \\\hline
   Expected for 36.1 \ifb  & $5.1\times 10^2$ \\
   $\geq 2$ SS leptons ($\pt>20 \GeV$)  & $19.96 \pm 0.35$ \\
   Trigger  & $19.17 \pm 0.35$ \\
   $\ge 2$ $b$-jets ($\pt>20 \GeV$)  & $16.10 \pm 0.32$ \\
   $\ge 6$ jets ($\pt>25 \GeV$)  & $13.11 \pm 0.28$ \\
   $\met>200 \GeV$  & $10.17 \pm 0.26$ \\
   $\meff>0.6 \TeV$  & $10.17 \pm 0.26$ \\
   $\met>0.25\times\meff$  & $5.94 \pm 0.20$ \\
\hline\end{tabular}
\caption{Number of signal events at different stages of the Rpc2L2bS signal region selection. 
Only statistical uncertainties are shown.}
\end{table}

\begin{table}[ht]\centering\def\arraystretch{1.2}\begin{tabular}{|l|c|}\hline
   \multicolumn{2}{|l|}{Rpc2L2bH,\quad$\gluino\gluino$ production,\quad$\gluino\to \ttbar\ninoone$}\\
   \multicolumn{2}{|l|}{$m_{\gluino}=1.7 \TeV$, $m_{\ninoone}=200 \GeV$}\\\hline
   MC events generated  & 98000 \\\hline
   Expected for 36.1 \ifb  & $1.7\times 10^2$ \\
   $\geq 2$ SS leptons ($\pt>20 \GeV$)  & $7.32 \pm 0.13$ \\
   Trigger  & $7.19 \pm 0.13$ \\
   $\ge 2$ $b$-jets ($\pt>20 \GeV$)  & $5.81 \pm 0.11$ \\
   $\ge 6$ jets ($\pt>40 \GeV$)  & $4.92 \pm 0.11$ \\
   $\meff>1.8 \TeV$  & $3.93 \pm 0.09$ \\
   $\met>0.15\times\meff$  & $3.12 \pm 0.08$ \\
\hline\end{tabular}
\caption{Number of signal events at different stages of the Rpc2L2bH signal region selection. 
Only statistical uncertainties are shown.}\end{table}

\begin{table}[ht]\centering\def\arraystretch{1.2}\begin{tabular}{|l|c|}\hline
   \multicolumn{2}{|l|}{Rpc2Lsoft1b,\quad$\gluino\gluino$ production,\quad$\gluino\to tWb\ninoone$}\\
   \multicolumn{2}{|l|}{$m_{\gluino}=1.2 \TeV$, $m_{\ninoone}=940 \GeV$}\\\hline
   MC events generated  & 50000 \\\hline
   Expected for 36.1 \ifb  & $3.1\times 10^3$ \\
   $\geq 2$ SS leptons ($100>\pt>20,10$~GeV)  & $101.9 \pm 2.7$ \\
   Trigger  & $89.3 \pm 2.5$ \\
   $\ge 1$ $b$-jet ($\pt>20 \GeV$)  & $75.1 \pm 2.3$ \\
   $\ge 6$ jets ($\pt>25 \GeV$)  & $31.5 \pm 1.5$ \\
   $\met>100 \GeV$  & $23.0 \pm 1.3$ \\
   $\met>0.3\times\meff$  & $6.5 \pm 0.7$ \\
\hline\end{tabular}
\caption{Number of signal events at different stages of the Rpc2Lsoft1b signal region selection. 
Only statistical uncertainties are shown.}\end{table}

\begin{table}[ht]\centering\def\arraystretch{1.2}\begin{tabular}{|l|c|}\hline
   \multicolumn{2}{|l|}{Rpc2Lsoft2b,\quad$\gluino\gluino$ production,\quad$\gluino\to tWb\ninoone$}\\
   \multicolumn{2}{|l|}{$m_{\gluino}=1.2 \TeV$, $m_{\ninoone}=900 \GeV$}\\\hline
   MC events generated  & 50000 \\\hline
   Expected for 36.1 \ifb  & $3.1\times 10^3$ \\
   $\geq 2$ SS leptons ($100>\pt>20,10$~GeV)  & $91.8 \pm 2.6$ \\
   Trigger  & $79.7 \pm 2.4$ \\
   $\ge 2$ $b$-jets ($\pt>20 \GeV$)  & $41.3 \pm 1.7$ \\
   $\ge 6$ jets ($\pt>25 \GeV$)  & $21.4 \pm 1.2$ \\
   $\met>200 \GeV$  & $8.7 \pm 0.7$ \\
   $\meff>0.6 \TeV$  & $8.7 \pm 0.7$ \\
   $\met>0.25\times\meff$  & $6.7 \pm 0.6$ \\
\hline\end{tabular}
\caption{Number of signal events at different stages of the Rpc2Lsoft2b signal region selection. 
Only statistical uncertainties are shown.}\end{table}

\begin{table}[ht]\centering\def\arraystretch{1.2}\begin{tabular}{|l|c|}\hline
   \multicolumn{2}{|l|}{Rpc2L0bS,\quad$\gluino\gluino$ production,\quad$\gluino\to q\bar q^{'}WZ\ninoone$}\\
   \multicolumn{2}{|l|}{$m_{\gluino}=1.2 \TeV$, $(m_{\chargino} - 150) = (m_{\tilde\chi_2^0} - 75) = m_{\ninoone}=900 \GeV$}\\\hline
   MC events generated  & 19000 \\\hline
   Expected for 36.1 \ifb  & $3.1\times 10^3$ \\
   $\geq 2$ SS leptons ($\pt>20 \GeV$)  & $64 \pm 4$ \\
   Trigger  & $58.6 \pm 3.3$ \\
   no $b$-jet ($\pt>20 \GeV$)  & $46.3 \pm 3.0$ \\
   $\ge 6$ jets ($\pt>25 \GeV$)  & $26.6 \pm 2.4$ \\
   $\met>150 \GeV$  & $16.3 \pm 2.0$ \\
   $\met>0.25\times\meff$  & $9.0 \pm 1.3$ \\
\hline\end{tabular}
\caption{Number of signal events at different stages of the Rpc2L0bS signal region selection. 
Only statistical uncertainties are shown.}\end{table}

\begin{table}[ht]\centering\def\arraystretch{1.2}\begin{tabular}{|l|c|}\hline
   \multicolumn{2}{|l|}{Rpc2L0bH,\quad$\gluino\gluino$ production,\quad$\gluino\to q\bar q^{'}WZ\ninoone$}\\
   \multicolumn{2}{|l|}{$m_{\gluino}=1.6 \TeV$, $(m_{\chargino} - 750) = (m_{\tilde\chi_2^0} - 375) = m_{\ninoone}=100 \GeV$}\\\hline
   MC events generated  & 20000 \\\hline
   Expected for 36.1 \ifb  & $2.9\times 10^2$ \\
   $\geq 2$ SS leptons ($\pt>20 \GeV$)  & $12.8 \pm 0.5$ \\
   Trigger  & $12.5 \pm 0.5$ \\
   no $b$-jet ($\pt>20 \GeV$)  & $8.5 \pm 0.4$ \\
   $\ge 6$ jets ($\pt>40 \GeV$)  & $7.12 \pm 0.35$ \\
   $\met>250 \GeV$  & $5.13 \pm 0.29$ \\
   $\meff>0.9 \TeV$  & $5.13 \pm 0.29$ \\
\hline\end{tabular}
\caption{Number of signal events at different stages of the Rpc2L0bH signal region selection. 
Only statistical uncertainties are shown.}\end{table}

\begin{table}[ht]\centering\def\arraystretch{1.2}\begin{tabular}{|l|c|}\hline
   \multicolumn{2}{|l|}{Rpc3L0bS,\quad$\gluino\gluino$ production,\quad$\gluino\to q\bar q(\tilde\ell\ell/\tilde\nu\nu)$}\\
   \multicolumn{2}{|l|}{$m_{\gluino}=1.4 \TeV$, $(m_{\tilde\chi_2^0} - 150) = (m_{\tilde\ell, \tilde\nu} - 75) = m_{\ninoone}=1100 \GeV$}\\\hline
   MC events generated  & 20000 \\\hline
   Expected for 36.1 \ifb  & $9.1\times 10^2$ \\
   $\geq 3$ leptons ($\pt>20,20,10$~GeV)  & $76.9 \pm 2.1$ \\
   Trigger  & $76.0 \pm 2.0$ \\
   no $b$-jet ($\pt>20 \GeV$)  & $67.5 \pm 1.9$ \\
   $\ge 4$ jets ($\pt>40 \GeV$)  & $31.6 \pm 1.3$ \\
   $\met>200 \GeV$  & $17.1 \pm 1.0$ \\
   $\meff>0.6 \TeV$  & $17.1 \pm 1.0$ \\
\hline\end{tabular}
\caption{Number of signal events at different stages of the Rpc3L0bS signal region selection. 
Only statistical uncertainties are shown.}\end{table}

\begin{table}[ht]\centering\def\arraystretch{1.2}\begin{tabular}{|l|c|}\hline
   \multicolumn{2}{|l|}{Rpc3L0bH,\quad$\gluino\gluino$ production,\quad$\gluino\to q\bar q(\tilde\ell\ell/\tilde\nu\nu)$}\\
   \multicolumn{2}{|l|}{$m_{\gluino}=1.8 \TeV$, $(m_{\tilde\chi_2^0} - 850) = (m_{\tilde\ell, \tilde\nu} - 375) = m_{\ninoone}=100 \GeV$}\\\hline
   MC events generated  & 20000 \\\hline
   Expected for 36.1 \ifb  & $1.0\times 10^{2}$ \\
   $\geq 3$ leptons ($\pt>20,20,10$~GeV)  & $9.98 \pm 0.25$ \\
   Trigger  & $9.94 \pm 0.25$ \\
   no $b$-jet ($\pt>20 \GeV$)  & $8.44 \pm 0.23$ \\
   $\ge 4$ jets ($\pt>40 \GeV$)  & $7.79 \pm 0.22$ \\
   $\met>200 \GeV$  & $6.58 \pm 0.21$ \\
   $\meff>1.6 \TeV$  & $6.56 \pm 0.21$ \\
\hline\end{tabular}
\caption{Number of signal events at different stages of the Rpc3L0bH signal region selection. 
Only statistical uncertainties are shown.}\end{table}

\begin{table}[ht]\centering\def\arraystretch{1.2}\begin{tabular}{|l|c|}\hline
   \multicolumn{2}{|l|}{Rpc2L1bS,\quad$\sbottomone\sbottomonebar$ production,\quad$\sbottomone\to t\tilde\chi_1^{-}\to t W^-
\ninoone$}\\
   \multicolumn{2}{|l|}{$m_{\sbottomone}=600 \GeV$, $m_{\chargino} = 350 \GeV$, $m_{\ninoone}=250 \GeV$}\\\hline
   MC events generated  & 10000 \\\hline
   Expected for 36.1 \ifb  & $6.3\times 10^3$ \\
   $\geq 2$ SS leptons ($\pt>20 \GeV$)  & $221 \pm 4$ \\
   Trigger  & $201 \pm 4$ \\
   $\ge 1$ $b$-jet ($\pt>20 \GeV$)  & $173 \pm 4$ \\
   $\ge 6$ jets ($\pt>25 \GeV$)  & $66.3 \pm 2.2$ \\
   $\met>150 \GeV$  & $36.5 \pm 1.7$ \\
   $\meff>0.6 \TeV$  & $36.1 \pm 1.7$ \\
   $\met>0.25\times\meff$  & $15.1 \pm 1.1$ \\
\hline\end{tabular}
\caption{Number of signal events at different stages of the Rpc2L1bS signal region selection. 
Only statistical uncertainties are shown.}\end{table}

\begin{table}[ht]\centering\def\arraystretch{1.2}\begin{tabular}{|l|c|}\hline
   \multicolumn{2}{|l|}{Rpc2L1bH,\quad$\sbottomone\sbottomonebar$ production,\quad$\sbottomone\to t\tilde\chi_1^{-}$}\\
   \multicolumn{2}{|l|}{$m_{\sbottomone}=750 \GeV$, $m_{\chargino} = 200 \GeV$, $m_{\ninoone}=100 \GeV$}\\\hline
   MC events generated  & 10000 \\\hline
   Expected for 36.1 \ifb  & $1.6\times 10^3$ \\
   $\geq 2$ SS leptons ($\pt>20 \GeV$)  & $71.1 \pm 1.2$ \\
   Trigger  & $66.4 \pm 1.2$ \\
   $\ge 1$ $b$-jet ($\pt>20 \GeV$)  & $56.6 \pm 1.1$ \\
   $\ge 6$ jets ($\pt>25 \GeV$)  & $27.7 \pm 0.7$ \\
   $\met>250 \GeV$  & $12.5 \pm 0.5$ \\
   $\met>0.2\times\meff$  & $9.5 \pm 0.4$ \\
\hline\end{tabular}
\caption{Number of signal events at different stages of the Rpc2L1bH signal region selection. 
Only statistical uncertainties are shown.}\end{table}

\begin{table}[ht]\centering\def\arraystretch{1.2}\begin{tabular}{|l|c|}\hline
   \multicolumn{2}{|l|}{Rpc3LSS1b,\quad$\stopone\stoponebar$ production,\quad$\stopone\to t\ninotwo\to \tilde t W^\pm \chi_1^\mp$}\\
   \multicolumn{2}{|l|}{$m_{\stopone}=700 \GeV$, $m_{\ninotwo}=525 \GeV$, $m_{\chargino}\approx m_{\ninoone}=425 \GeV$}\\\hline
   MC events generated  & 5000 \\\hline
   Expected for 36.1 \ifb  & $2.4\times 10^3$ \\
   $\geq 3$ SS leptons ($\pt>20,20,10$~GeV), $Z\to e^\pm e^\pm$ veto  & $4.6 \pm 0.5$ \\
   Trigger  & $4.5 \pm 0.5$ \\
   $\ge 1$ $b$-jet ($\pt>20 \GeV$)  & $3.6 \pm 0.4$ \\
\hline\end{tabular}
\caption{Number of signal events at different stages of the Rpc3LSS1b signal region selection. 
Only statistical uncertainties are shown.}\end{table}

\begin{figure}[ht]
\centering
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/acceptance_2StepRpc2L0bH}\caption{Rpc2L0bH acceptance}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/efficiency_2StepRpc2L0bH}\caption{Rpc2L0bH efficiency}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/acceptance_2StepRpc2L0bS}\caption{Rpc2L0bS acceptance}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/efficiency_2StepRpc2L0bS}\caption{Rpc2L0bS efficiency}\end{subfigure}
\caption{Signal acceptance (a,c) and reconstruction efficiency (b,d) 
for simplified models of $\gluino\gluino$ production with $\gluino\to q\bar q^{'}WZ\ninoone$ decays, 
in the signal regions Rpc2L0bH (a,b) and Rpc2L0bS (c,d).}
\end{figure}

\begin{figure}[ht]
\centering
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/acceptance_GSLRpc3L0bH}\caption{Rpc3L0bH acceptance}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/efficiency_GSLRpc3L0bH}\caption{Rpc3L0bH efficiency}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/acceptance_GSLRpc3L0bS}\caption{Rpc3L0bS acceptance}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/efficiency_GSLRpc3L0bS}\caption{Rpc3L0bS efficiency}\end{subfigure}
\caption{Signal acceptance (a,c) and reconstruction efficiency (b,d) 
for simplified models of $\gluino\gluino$ production with $\gluino\to q\bar q(\ell\ell/\nu\nu)\ninoone$ decays, 
in the signal regions Rpc3L0bH (a,b) and Rpc3L0bS (c,d).}
\end{figure}

\begin{figure}[ht]
\centering
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/acceptance_GttRpc2L2bH}\caption{Rpc2L2bH acceptance}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/efficiency_GttRpc2L2bH}\caption{Rpc2L2bH efficiency}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/acceptance_GttRpc2L2bS}\caption{Rpc2L2bS acceptance}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/efficiency_GttRpc2L2bS}\caption{Rpc2L2bS efficiency}\end{subfigure}
\caption{Signal acceptance (a,c) and reconstruction efficiency (b,d) 
for simplified models of $\gluino\gluino$ production with $\gluino\to t\bar t\ninoone$ decays, 
in the signal regions Rpc2L2bH (a,b) and Rpc2L2bS (c,d).}
\end{figure}

\begin{figure}[ht]
\centering
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/acceptance_GttRpc2Lsoft1b}\caption{Rpc2Lsoft1b acceptance}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/efficiency_GttRpc2Lsoft1b}\caption{Rpc2Lsoft1b efficiency}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/acceptance_GttRpc2Lsoft2b}\caption{Rpc2Lsoft2b acceptance}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/efficiency_GttRpc2Lsoft2b}\caption{Rpc2Lsoft2b efficiency}\end{subfigure}
\caption{Signal acceptance (a,c) and reconstruction efficiency (b,d) 
for simplified models of $\gluino\gluino$ production with $\gluino\to t\bar t\ninoone$ decays, 
in the signal regions Rpc2Lsoft1b (a,b) and Rpc2Lsoft2b (c,d).}
\end{figure}

\begin{figure}[ht]
\centering
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/acceptance_ComprGttRpc2L2bH}\caption{Rpc2L2bH acceptance}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/efficiency_ComprGttRpc2L2bH}\caption{Rpc2L2bH efficiency}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/acceptance_ComprGttRpc2L2bS}\caption{Rpc2L2bS acceptance}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/efficiency_ComprGttRpc2L2bS}\caption{Rpc2L2bS efficiency}\end{subfigure}
\caption{Signal acceptance (a,c) and reconstruction efficiency (b,d) 
for simplified models of $\gluino\gluino$ production with $\gluino\to tWb\ninoone$ decays (region with $\Delta m(\gluino,\ninoone)<2m_t$), 
in the signal regions Rpc2L2bH (a,b) and Rpc2L2bS (c,d).}
\end{figure}

\begin{figure}[ht]
\centering
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/acceptance_ComprGttRpc2Lsoft1b}\caption{Rpc2Lsoft1b acceptance}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/efficiency_ComprGttRpc2Lsoft1b}\caption{Rpc2Lsoft1b efficiency}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/acceptance_ComprGttRpc2Lsoft2b}\caption{Rpc2Lsoft2b acceptance}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/efficiency_ComprGttRpc2Lsoft2b}\caption{Rpc2Lsoft2b efficiency}\end{subfigure}
\caption{Signal acceptance (a,c) and reconstruction efficiency (b,d) 
for simplified models of $\gluino\gluino$ production with $\gluino\to tWb\ninoone$ decays (region with $\Delta m(\gluino,\ninoone)<2m_t$), 
in the signal regions Rpc2Lsoft1b (a,b) and Rpc2Lsoft2b (c,d).}
\end{figure}

\begin{figure}[ht]
\centering
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/acceptance_BttRpc2L1bH}\caption{Rpc2L1bH acceptance}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/efficiency_BttRpc2L1bH}\caption{Rpc2L1bH efficiency}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/acceptance_BttRpc2L1bS}\caption{Rpc2L1bS acceptance}\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\includegraphics[width=\textwidth]{EffAcc/efficiency_BttRpc2L1bS}\caption{Rpc2L1bS efficiency}\end{subfigure}
\caption{Signal acceptance (a,c) and reconstruction efficiency (b,d) 
for simplified models of $\sbottomone\sbottomonebar$ production with $\sbottomone\to tW^{-}\ninoone$ decays, 
in the signal regions Rpc2L1bH (a,b) and Rpc2L1bS (c,d).}
\end{figure}


\begin{table}[ht]\centering\begin{tabular}{|l|c|c|c|c|c|c|c|}\hline
\multicolumn{8}{|l|}{Rpc2L2bH,\quad $\gluino\gluino$ production in the NUHM2 model}\\\hline
$m_{\gluino}$ [GeV] & 300 & 350 & 400 & 500 & 600 & 700 & 800 \\\hline
Acceptance & 0.8\% & 1.6\% & 2.1\% & 3.2\% & 3.5\% & 4.4\% & 4.0\% \\
Efficiency & 43\% & 49\% & 50\% & 49\% & 48\% & 43\% & 49\%\\\hline
\end{tabular}
\caption{Rpc2L2bH signal region acceptance and reconstruction efficiency for $\gluino\gluino$ production in the NUHM2 model.}
\end{table}

\begin{table}[ht]\centering\begin{tabular}{|l|c|c|c|c|c|c|}\hline
\multicolumn{7}{|l|}{Rpc3LSS1b,\quad $\stopone\stoponebar$ production,\quad $\stopone\to t\ninotwo$, $\ninotwo\to W^\mp\chargino$}\\\hline
$m_{\stopone}$ [GeV] & 550 & 600 & 650 & 700 & 750 & 800 \\\hline
Acceptance & 0.3\% & 0.3\% & 0.3\% & 0.4\% & 0.4\% & 0.4\%\\
Efficiency & 36\% & 42\% & 44\% & 37\% & 33\% & 30\%\\\hline
\end{tabular}
\caption{Rpc3LSS1b signal region acceptance and reconstruction efficiency for $\stopone\stoponebar$ production with $\stopone\to t\ninotwo$ ($\ninotwo\to W\chargino$) decays.}
\end{table}


==> texfiles/app.bkg.dist.tex <==

\begin{figure}[t!]
\centering
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{EE_2JMET50_meff}
\caption{Effective mass \meff}
\end{subfigure}
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{EE_2JMET50_met}
\caption{Missing transverse momentum \met}
\end{subfigure}
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{EE_2JMET50_njets25}
\caption{Number of jets ($\pt>25~\GeV$)}
\end{subfigure}
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{EE_2JMET50_nbjets}
\caption{Number of $b$-tagged jets ($\pt>20~\GeV$)}
\end{subfigure}
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{EE_2JMET50_subSS_Pt}
\caption{Subleading SS lepton \pt}
\end{subfigure}
\caption{Di-electron channel: comparisons between observed data (2015+2016, 36 \ifb) and expected SM+detector backgrounds 
for events with $\ge 2$ same-sign leptons ($\pt>20~\GeV$), $\met>50~\GeV$ and $\ge 2$ jets ($\pt>40~\GeV$). 
Uncertainties include statistical sources, as well as systematic uncertainties for the data-driven backgrounds; 
for illustration, statistical uncertainties alone are shown in the light-colored error bands in the ratio plots. 
Events belonging to any of the signal regions are rejected, both in data and MC. 
}
\label{fig:distributions_channelEE_2015}
\end{figure} 

\begin{figure}[t!]
\centering
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{EM_2JMET50_meff}
\caption{Effective mass \meff}
\end{subfigure}
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{EM_2JMET50_met}
\caption{Missing transverse momentum \met}
\end{subfigure}
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{EM_2JMET50_njets25}
\caption{Number of jets ($\pt>25~\GeV$)}
\end{subfigure}
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{EM_2JMET50_nbjets}
\caption{Number of $b$-tagged jets ($\pt>20~\GeV$)}
\end{subfigure}
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{EM_2JMET50_subSS_Pt}
\caption{Subleading SS lepton \pt}
\end{subfigure}
\caption{Electron-muon channel: comparisons between observed data (2015+2016, 36 \ifb) and expected SM+detector backgrounds 
for events with $\ge 2$ same-sign leptons ($\pt>20~\GeV$), $\met>50~\GeV$ and $\ge 2$ jets ($\pt>40~\GeV$). 
Uncertainties include statistical sources, as well as systematic uncertainties for the data-driven backgrounds; 
for illustration, statistical uncertainties alone are shown in the light-colored error bands in the ratio plots. 
Events belonging to any of the signal regions are rejected, both in data and MC.  
}
\label{fig:distributions_channelEM_2015}
\end{figure} 

\begin{figure}[t!]
\centering
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{MM_2JMET50_meff}
\caption{Effective mass \meff}
\end{subfigure}
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{MM_2JMET50_met}
\caption{Missing transverse momentum \met}
\end{subfigure}
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{MM_2JMET50_njets25}
\caption{Number of jets ($\pt>25~\GeV$)}
\end{subfigure}
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{MM_2JMET50_nbjets}
\caption{Number of $b$-tagged jets ($\pt>20~\GeV$)}
\end{subfigure}
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{MM_2JMET50_subSS_Pt}
\caption{Subleading SS lepton \pt}
\end{subfigure}
\caption{Di-muon channel: comparisons between observed data (2015+2016, 36 \ifb) and expected SM+detector backgrounds 
for events with $\ge 2$ same-sign leptons ($\pt>20~\GeV$), $\met>50~\GeV$ and $\ge 2$ jets ($\pt>40~\GeV$). 
Uncertainties include statistical sources, as well as systematic uncertainties for the data-driven backgrounds; 
for illustration, statistical uncertainties alone are shown in the light-colored error bands in the ratio plots. 
Events belonging to any of the signal regions are rejected, both in data and MC.  
}
\label{fig:distributions_channelMM_2015}
\end{figure} 

\begin{figure}[t!]
\centering
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{TRILEP_2JMET50_meff}
\caption{Effective mass \meff}
\end{subfigure}
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{TRILEP_2JMET50_met}
\caption{Missing transverse momentum \met}
\end{subfigure}
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{TRILEP_2JMET50_njets25}
\caption{Number of jets ($\pt>25~\GeV$)}
\end{subfigure}
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{TRILEP_2JMET50_nbjets}
\caption{Number of $b$-tagged jets ($\pt>20~\GeV$)}
\end{subfigure}
\begin{subfigure}[t]{0.48\textwidth}
\includegraphics[width=\textwidth]{TRILEP_2JMET50_subSS_Pt}
\caption{Subleading SS lepton \pt}
\end{subfigure}
\caption{Trilepton channel: comparisons between observed data (2015+2016, 36 \ifb) and expected SM+detector backgrounds 
for events with $\ge 3$ leptons ($\pt>20~\GeV$ for the two leading leptons, $\pt>10~\GeV$ for the third lepton), $\met>50~\GeV$ and $\ge 2$ jets ($\pt>40~\GeV$). 
Uncertainties include statistical sources, as well as systematic uncertainties for the data-driven backgrounds; 
for illustration, statistical uncertainties alone are shown in the light-colored error bands in the ratio plots. 
Events belonging to any of the signal regions are rejected, both in data and MC.  
}
\label{fig:distributions_channel3L_2015}
\end{figure} 


==> texfiles/app.hf.tex <==
Ex%%amples of one of some signal region with the breakdown of systematic uncertainties  produced with the \texttt{HistFitter} framework.


% Systematics tables
%%\input{texfiles/HFtables/SystBgOnlyRpc2L0bH}
%% \input{texfiles/HFtables/SystBgOnlyRpc2L0bS}
%% \input{texfiles/HFtables/SystBgOnlyRpc2L1bH}
%% \input{texfiles/HFtables/SystBgOnlyRpc2L1bS}
%% \input{texfiles/HFtables/SystBgOnlyRpc2L2bH}
%% \input{texfiles/HFtables/SystBgOnlyRpc2L2bS}
%% \input{texfiles/HFtables/SystBgOnlyRpc2Lsoft1b}
%% \input{texfiles/HFtables/SystBgOnlyRpc2Lsoft2b}
%% \input{texfiles/HFtables/SystBgOnlyRpc3L0bH}
%% \input{texfiles/HFtables/SystBgOnlyRpc3L0bS}
%% \input{texfiles/HFtables/SystBgOnlyRpc3L1bH}
%% \input{texfiles/HFtables/SystBgOnlyRpc3L1bS}
%% \input{texfiles/HFtables/SystBgOnlyRpc3LSS1b}


==> texfiles/subsec.bkg.comp.tex <==
The MC template method is validated by looking at the Data/MC agreement near the signal regions where we invert one of the cuts while keeping the last bin corresponding to the SR blinded. 
These distributions can be found in Figure~\ref{app:mctemplate}.


==> texfiles/subsec.bkg.res.tex <==
The expected yield for processes with FNP leptons, 
estimated with the method described in 
Sections~\ref{sec:bkg.red.mct} and~\ref{subsec:fakes_mctemplate}, 
are presented in Table~\ref{tab:fakes_sr_yields} for the signal regions. 
The estimates are all found to be consistent with each other. 

The final numbers retained for the fake lepton background estimate,
shown in Table~\ref{tab:fakes_sr_yields}
are taken as the weighted-average of the predictions from the matrix method 
and the MC template; 
the weights are based on the statistical component, and the systematic 
uncertainties are propagated 
assuming conservatively a full correlation between the two methods, 
although they are in fact largely independent. 
The central value along with the statistical and systematic uncertainties 
are therefore: 

\begin{equation}
\begin{aligned}
& \left(w\zeta_1 + (1-w)\zeta_2\right) 
\pm \sqrt{w^2\left(\Delta\zeta_1^\text{(stat)}\right)^2 + (1-w)^2\left(\Delta\zeta_2^\text{(stat)}\right)^2} \\
&\hspace{3.225cm} \pm \left(w\Delta\zeta_1^\text{(syst)} + (1-w)\Delta\zeta_2^\text{(syst)}\right)\\
&\qquad\text{ with }w=\frac{\left(\Delta\zeta_2^\text{(stat)}\right)^2}{\left(\Delta\zeta_1^\text{(stat)}\right)^2+\left(\Delta\zeta_2^\text{(stat)}\right)^2}\notag
\end{aligned}
\end{equation}

When the estimated value is too small (below 0.15), the expected yield is set
 to $0.15\pm 0.15$, 
to cover for possibilities of an under-fluctuation of the number of
 baseline-not-signal leptons 
when applying the matrix method, as well as lack of statistics in the MC 
samples for the other method. 

\begin{table}[!htb]
  \caption{Expected yields for background processes with FNP leptons
    shown for 36 \ifb. Uncertainties include all statistical and systematic 
sources for the nominal estimate . 
}
\label{tab:fakes_sr_yields}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||c|c||c|}\hline
      Region &              Matrix method   &   Template method   &     Retained estimate  \\\hline
    Rpc2L0bH & $ 0.83 \pm  0.56 \pm  0.74$  &  $1.00 \pm 0.96 \pm 0.81$ &  $ 0.87 \pm  0.48 \pm  0.76$  \\
    Rpc2L0bS & $ 1.51 \pm  0.60 \pm  0.66$  &  $1.68 \pm 1.02 \pm 1.26$  &  $ 1.55 \pm  0.52 \pm  0.81$  \\
    Rpc2L1bH & $ 3.54 \pm  1.62 \pm  3.12$  &  $2.07 \pm 0.63 \pm 1.56$  &  $ 2.26 \pm  0.59 \pm  1.76$  \\
    Rpc2L1bS & $ 2.65 \pm  1.21 \pm  1.89$  &  $02.33 \pm 01.17 \pm 02.10$  & $ 2.48 \pm  0.84 \pm  2.00$  \\ 
    Rpc2L2bH & $-0.11 \pm  0.11 \pm  0.18$  &  $<0.5$  &  $ 0.15 \pm  0.15 \pm  0.00$  \\
    Rpc2L2bS & $ 1.31 \pm  1.07 \pm  1.65$  &  $0.41 \pm 0.33 \pm 0.45$ &  $ 0.49 \pm  0.32 \pm  0.55$  \\
    Rpc2Lsoft1b & $ 4.75 \pm  1.42 \pm  2.64$  &  $2.48 \pm 1.32 \pm 1.86$  &  $ 3.53 \pm  0.97 \pm  2.22$  \\
    Rpc2Lsoft2b & $ 1.91 \pm  1.18 \pm  1.63$  &  $1.66 \pm 0.66 \pm 1.28$ &  $ 1.72 \pm  0.58 \pm  1.36$  \\
    Rpc3L0bH & $-0.01 \pm  0.11 \pm  0.10$  &  $<0.5$                     &  $ 0.15 \pm  0.15 \pm  0.00$  \\
    Rpc3L0bS & $ 2.31 \pm  1.50 \pm  2.63$  &  $0.21 \pm 0.15 \pm 0.16$   &  $ 0.23 \pm  0.15 \pm  0.18$  \\
    Rpc3L1bH & $ 0.57 \pm  0.43 \pm  0.50$  &  $0.42 \pm 0.29 \pm 0.32$  
                      &  $ 0.47 \pm  0.24 \pm  0.38$  \\
    Rpc3L1bS & $ 4.94 \pm  1.83 \pm  2.96$  &  $3.55 \pm 1.80 \pm 2.76$   &  $ 4.23 \pm  1.28 \pm  2.86$  \\
    Rpc3LSS1b & $-0.18 \pm  1.24 \pm  2.85$  &  $0.90 \pm 0.14 \pm 0.69$  
    &  $ 0.89 \pm  0.14 \pm  0.72$  \\
\hline
\hline
\end{tabular}
}
\end{table}


\begin{figure}[htb!]
\centering
\begin{subfigure}[t]{0.66\textwidth}\includegraphics[width=\textwidth]{ETA_SS_BDTEL}\end{subfigure}
\caption{Invariant mass of the signal $e^{\pm} e^{\pm}$ pair distribution with (full markers) and without (open markers) charge-flip electron BDT selection applied.
}
\label{fig:ETA_SS_BDTEL}
\end{figure}



\begin{table}[!htb]
\caption{Expected yields for background processes with charge-flipped electrons
in the signal regions. Comparison between the data-driven and the MC template
estimates.
Uncertainties include all statistical and systematic sources. 
Charge-flip processes do not contribute to signal regions which require $\ge 3$ leptons. 
}
\label{tab:chargeflip_sr_yields}
\centering
\begin{tabular}{|c||c|c|}\hline
 Region      &   Weighted OS data          &     Template method \\\hline
    Rpc2L0bH & $ 0.01 \pm  0.00 \pm  0.00$ & $<0.4$ \\
    Rpc2L0bS & $ 0.05 \pm  0.01 \pm  0.01$ & $ 00.02 \pm 00.02 \pm 00.00 $ \\
    Rpc2L1bH & $ 0.25 \pm  0.03 \pm  0.04$ & $ 00.21 \pm 00.32 \pm 00.16 $ \\
    Rpc2L1bS & $ 0.25 \pm  0.02 \pm  0.04$ & $ 00.35 \pm 00.37 \pm 00.26 $ \\
    Rpc2L2bH & $ 0.02 \pm  0.01 \pm  0.00$ & $<0.4$ \\
    Rpc2L2bS & $ 0.10 \pm  0.01 \pm  0.02$ & $<0.4$ \\
 Rpc2Lsoft1b & $ 0.08 \pm  0.01 \pm  0.02$ & $<0.4$ \\
 Rpc2Lsoft2b & $ 0.08 \pm  0.01 \pm  0.02$ & $<0.4$ \\
   Rpc3LSS1b & $ 0.39 \pm  0.03 \pm  0.07$ & $ 00.81 \pm 00.53 \pm 00.34 $ \\
\hline
\hline
\end{tabular}
\end{table}

